Scenario-Based Trajectory Optimization in Uncertain Dynamic Environments

We present an optimization-based method to plan the motion of an autonomous robot under the uncertainties associated with dynamic obstacles, such as humans. Our method bounds the marginal risk of collisions at each point in time by incorporating chance constraints into the planning problem. This problem is not suitable for online optimization outright for arbitrary probability distributions. Hence, we sample from these chance constraints using an uncertainty model, to generate "scenarios", which translate the probabilistic constraints into deterministic ones. In practice, each scenario represents the collision constraint for a dynamic obstacle at the location of the sample. The number of theoretically required scenarios can be very large. Nevertheless, by exploiting the geometry of the workspace, we show how to prune most scenarios before optimization and we demonstrate how the reduced scenarios can still provide probabilistic guarantees on the safety of the motion plan. Since our approach is scenario based, we are able to handle arbitrary uncertainty distributions. We apply our method in a Model Predictive Contouring Control framework and demonstrate its benefits in simulations and experiments with a moving robot platform navigating among pedestrians, running in real-time.

==> content/theoretical_results.tex <==
\section{Theoretical Results}\label{sec:proofs}
{\textcolor{red}{ in method or problem formulation!}}
We collect the samples of each stage as multi-samples for each stage as $\bm{\omega}_k = \{\bm{\delta}_k^1, \hdots \bm{\delta}_k^{S_k}\}$. The following assumption is necessary:\\

\begin{assumption}\label{as:sampling}
The set formed by the scenarios and the real uncertainty per stage,
\begin{equation}
    \bm{\omega}_k \cup \bm{\delta}_k, \quad \bm{\delta}_k \in \Delta_k,\label{eq:as}
\end{equation}
is independent and identically distributed (iid) for all $k$.
\end{assumption}

\subsection{Scenario Optimization with Multiple Chance Constraints}
In the following, we show that under Assumption \ref{as:sampling}, scenario theory may be applied to multiple chance constraints. The proof is analogous to the convex proof presented in \cite[Theorem Fix]{schildbach}.

\begin{proof}[Proof of Theorem \ref{theory:per_stage}]
In the following, we derive the result for $k=1$. The proof is analogous for all other $k$. Consider the violation probability of the first stage, 
\begin{equation}
    \mathbb{P}[V_1(\b{u}^*) > \epsilon_1(s_1^*) \ | \ \bm{\omega}_2, \hdots \bm{\omega}_N ],
\end{equation}
i.e., the probability of drawing a multi-sample $\bm{\omega}_1$, such that the violation probability of $\b{x}^*$ exceeds $\epsilon_1$, when $\bm{\omega}_2, \hdots \bm{\omega}_N$ are known. By assumption \ref{as:sampling}, the samples $\bm{\omega_1}$ are independent of the samples drawn for other stages. Moreover, since $\bm{\omega}_2, \hdots \bm{\omega}_N$ are deterministic, we can merge their respective constraints into the feasible set
\begin{equation}
    \Tilde{\mathbb{X}}^1 =  \bigcap_{k = 2}^N \{\b{x}_k \ | \ g(\b{x}_k, \bm{\omega}_k) \leq 0 \}.
\end{equation}
This results in the following modified optimisation problem
\begin{subequations}
\begin{align}
    \min_{\b{u} \in \mathbb{U}} \qquad & \sum_{k = 1}^N J(\b{x}_k, \b{u}_k)\\
  \textrm{s.t.} \qquad & \b{x}_{k + 1} = f(\b{x}_k, \b{u}_k) \\
   &\mathbb{P}[ \ ||\b{x}_1 - \bm{\delta}_1||_2 > r] \geq 1 - \epsilon_1 \\
   &\b{x}_{2:N} \in \Tilde{\mathbb{X}}^1\label{eq:ccp_multistage_1}
\end{align}
\end{subequations}
This problem is a nonconvex CCP of the form \eqref{eq:ccp}. The support subsample $s_1$, risk $\epsilon_1$ and violation probability $\beta_1$ at the first stage are therefore related by
\begin{equation}
    \mathbb{P} [V_1(\b{u}^*) > \epsilon_1(s_1^*) \ | \ \bm{\omega}_2, \hdots \bm{\omega}_N ] \leq \beta, 
\end{equation}
with
\begin{equation}
    \sum_{k = 0}^{S_1 - 1} {S_1 \choose k}(1 - \epsilon_1(k))^{S_1 - k} = \beta.
\end{equation}
The same derivations hold for $k = 2, \hdots, N$, which completes the proof.
\end{proof}


% Relevant! but should not be here
%In this separated formulation, the support subsample and the sampling size are stage specific. Hence it is possible to allocate risk among stages by adjusting $\epsilon_k$, resulting in different sampling sizes $S_k$. This allows us to discount future stages specifically, which yield feasible planners even if future predictions are highly uncertain.

\subsection{A Posteriori Scenario Discarding}
% Scenario sampling from long-tailed distributions may be conservative, since the worst samples result in the tightest constraints. The bounds that these scenarios set are often far from the specified safety level. We consider in the following to discard the worst samples in terms of performance, at the cost of sampling more points initially, similarly to the approached followed by \cite{campi_sampling-and-discarding_2011} for the convex case.\\

In the following proof we show that after discarding, the problem reduces to a smaller sized scenario problem. By noting that discarding is a binomial process, we obtain an upper bound for the violation probability. We define a discarding algorithm $\mathcal{P}$ that discards $R$ scenarios out of $S$ scenarios after sampling. The remaining $P = S - R$ scenarios are considered in the optimization.

\begin{theorem}
Let $\epsilon(k)$ be a function such that
\begin{align*}
    &\epsilon(P) = 1\\
    &{S \choose P}\sum_{k=0}^{P-1}{P \choose k}(1- \epsilon(k))^{P-k} = \beta.
\end{align*}
Let $\mathcal{P}$ remove $R$ scenarios a posteriori. Then the violation probability is bounded by
\begin{equation}
    \mathbb{P}[V(\b{u}^*) > \epsilon(s)] \leq\beta.
\end{equation}
\end{theorem}


\begin{proof}
Consider the following partitioning of the probability space:
\begin{equation}
    \Delta^S_{\mathcal{I}_p} = \{\bm{\delta}^S \in \Delta^S \ | \ \mathcal{P}(\bm{\delta}^S) = \mathcal{I}_p\},
\end{equation}
The sets $\Delta^S_{\mathcal{I}_p}$ are events where the picking algorithm selected the indices $\mathcal{I}_p$. Along the same lines we can define the set of violations as
\begin{equation}
    \mathcal{B} = \{\bm{\delta}^S \ | \mathcal{P}(\bm{\delta}^S) = \mathcal{I}_p, V(\b{x}_p^*) > \epsilon(s_p^*) \}.
\end{equation}
For exemplification, we now consider one specific index set, the set $\mathcal{I}_p = \{0, \hdots, P-1\}$. Its violation probability is
\begin{equation}
    \mathcal{B}_{ \{0, \hdots, P-1\}}= \{\bm{\delta}^S \ | \mathcal{P}(\bm{\delta}^S) = \mathcal{I}_{\{0, \hdots, P-1\}}, V(\b{x}_p^*) > \epsilon(s_p^*) \}.
\end{equation}
The definition of this violation set depends only on the picked samples. In fact the last condition is upper bounded by \cite[Theorem 1]{campi_general_2018}, where the sample size is replace with the picked scenario size.

Since $\mathcal{P}$ is deterministic, this probability is a cylinder with base in $\Delta^{S - P}$. The violation probability with these picked indices is in fact an instance of non-convex scenario optimisation on a limited probability space $\Tilde{\Delta} \subset \Delta$, but since the probability space is irrelevant for scenario theory, it follows that we can apply the seminal results directly. I.e., the probability of violation when index set $\mathcal{I}_p$ was picked is bounded by
\begin{equation}
    \mathbb{P}^P[\mathcal{B}_{ \{0, \hdots, P-1\}}] \leq \sum_{k=0}^{P-1}{P \choose k}(1- \epsilon(k))^{P-k} = \beta
\end{equation}
Since the index set $\{0, \hdots, P-1\}$ was picked arbitrarily, we obtain the same result for all other index sets. Hence the probability of violation with discarding can be upper bounded by
\begin{align}
    \mathbb{P}\{\mathcal{B}\} &= \bigcup_{\mathcal{I}_p} \mathbb{P}^P\{\mathcal{B}_{\mathcal{I}_p} \}\\
     &\leq  \bigcup_{\mathcal{I}_p} \sum_{k=0}^{P-1}{P \choose k}(1- \epsilon(k))^{P-k}\\
     &= {S \choose P}\sum_{k=0}^{P-1}{P \choose k}(1- \epsilon(k))^{P-k} = \beta
\end{align}
\end{proof}

%\begin{corollary}\label{col:eps}
We can define $\epsilon(k)$ as
\begin{equation}
    \epsilon(k) = 1 - \sqrt[P - k]{\frac{\beta}{{S \choose P} s_k {P \choose k}}},\label{eq:eps_discard}
\end{equation}
Figure \ref{fig:nonconvex_sizes} shows this function for varying values of $S$ and $R = S-P$.\\

Equation \eqref{eq:eps_discard} easily runs into numerical problems. To still compute it, we can split-up the binomial expressions, using the identity:
\begin{equation}
    {S \choose P} = {S \choose P-1} \frac{S - (P - 1)}{P}.
\end{equation}
Using this identity we can apply the root in between steps, leading to the computations of the form
\begin{equation*}
        \sqrt[P - k]{\frac{\beta}{{S \choose P}}}= \sqrt[P - k]{\frac{\beta}{\frac{S}{1}}} \sqrt[P - k]{\frac{\beta}{\frac{S-1}{2}}} \hdots \sqrt[P - k]{\frac{\beta}{\frac{S-(P-1)}{P}}}\\
\end{equation*}
%\end{corollary}

% \begin{figure}[h!]
%      \centering
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/simulation/discarding_sigma1_R0.eps}
%          \caption{$R = 0$}
%          \label{fig:r0}
%      \end{subfigure}
%      \newline
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/simulation/discarding_sigma1_R5.eps}
%          \caption{$R = 5$}
%          \label{fig:r5}
%      \end{subfigure}
%      \newline
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/simulation/discarding_sigma1_R10.eps}
%          \caption{$R = 10$}
%          \label{fig:r10}
%      \end{subfigure}
%      \newline
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/simulation/discarding_sigma1_R15.eps}
%          \caption{$R = 15$}
%          \label{fig:r15}
%      \end{subfigure}
%     \label{fig:removal_gaussian}
%      \caption{An example for scenario discarding in 1D. The selected scenario improves for more removals but does not surpass the bound.}
% \end{figure}
% NICER HERE IS FIGURES WITH SMALL HEIGHT 4 BELOW EACH OTHER!
% Also plot the variance of the beta comparison
\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figures/simulation/beta_comparison.eps}
\caption{Conservatism of the selected constraint over different values of the confidence parameter $\beta$ for a 1D Gaussian toy example.}
\label{fig:beta_gaussian}
\end{figure}
% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.75\textwidth]{Nonconvex_with_removal.eps}
% \caption{Safety level $\epsilon$ for varying sample size $S$ and scenario removal size $R$. The support subsample is assumed constant at $s_k = k = 4$.}
% \label{fig:nonconvex_sizes}
% \end{figure}
